VFLIP: A Backdoor Defense for Vertical Federated Learning via Identification and Purification

Vertical Federated Learning (VFL) focuses on handling vertically partitioned data over FL participants. Recent studies have discovered a significant vulnerability in VFL to backdoor attacks which specifically target the distinct characteristics of VFL. Therefore, these attacks may neutralize existing defense mechanisms designed primarily for Horizontal Federated Learning (HFL) and deep neural networks. In this paper, we present the first backdoor defense, called VFLIP, specialized for VFL. VFLIP employs the identification and purification techniques that operate at the inference stage, consequently improving the robustness against backdoor attacks to a great extent. VFLIP first identifies backdoor-triggered embeddings by adopting a participant-wise anomaly detection approach. Subsequently, VFLIP conducts purification which removes the embeddings identified as malicious and reconstructs all the embeddings based on the remaining embeddings. We conduct extensive experiments on CIFAR10, CINIC10, Imagenette, NUS-WIDE, and BankMarketing to demonstrate that VFLIP can effectively mitigate backdoor attacks in VFL. https://github.com/blingcho/VFLIP-esorics24

==> tables/datasets.tex <==
{
\resizebox{0.7\linewidth}{!}{
\def\arraystretch{1.0}
\begin{tabular}{ccccccc}
\toprule
Dataset    & Classes & Train & Val & Test  & Aux & Dim       \\ 
\midrule
CIFAR10    & 10      & 49500  & 500&9800  & 200 & 3$\times$32$\times$32   \\ 
\midrule
CINIC10    & 10      & 89100  &900& 89800 & 200 & 3$\times$32$\times$32     \\ 
\midrule
Imagenette & 10      & 9375  &94 & 3825  & 200 & 3$\times$224$\times$224   \\
\midrule
NUS-WIDE         & 5       & 25740 & 260& 6200 & 300  & 1634        \\ 
\midrule
BM & 2      & 53749  &540 & 53989  & 500 & 40   \\

\bottomrule

\end{tabular}
}
}

==> tables/default.tex <==
{
\resizebox{0.7\linewidth}{!}{
\def\arraystretch{1.0}
\begin{tabular}{ccccc}
\toprule
Dataset    & Learning Rate & Batch Size & Epochs &  Model Arch  \\ 
\midrule
CIFAR10    & 0.1           & 128        & 50                          & VGG19       \\ 
\midrule
CINIC10    & 0.1           & 128        & 50                          & VGG19       \\ 
\midrule
Imagenette & 0.1           & 128         & 50                         & VGG19       \\ 
\midrule

NUS-WIDE         & 0.1           & 256        & 50                          & 4-layer FCN \\
\midrule

BM & 0.1           & 128         & 40             & 4-layer FCN       \\ 

\bottomrule
\end{tabular}
}
}

==> tables/dpsgd_params.tex <==
{\Large
% \resizebox{0.7\textwidth}{!}{
\resizebox{\linewidth}{!}{
\def\arraystretch{1.1}
\begin{tabular}{ccccc}
\toprule
Dataset    & Clipping Bound ($C$) & Noise Scale ($\sigma$) & Privacy Loss ($\epsilon$) & Accuracy ($\%$) \\ 
\midrule


\multirow{5}{*}{\makecell{\\ \\ \\CIFAR10 }}&
\multirow{5}{*}{\makecell{\\ \\ \\ 0.4  }}&

10      & 3.64    & 10.00  \\  
&& 8    & 4.65    & 10.00  \\  
&& 6    & 6.35    & 77.74  \\  
&& 5    & 7.84    & 78.12  \\  
&& 4    & 10.09    & 77.08  \\  
&& 3    & 14.09    & 78.31  \\  
&& 2    & 24.01    & 78.25  \\  
&& 1    & 61.51    & 78.35  \\ 

\midrule

\multirow{5}{*}{\makecell{\\ \\ \\CINIC10 }}&
\multirow{5}{*}{\makecell{\\ \\ \\ 0.5  }}&

10      & 3.64    & 10.00  \\  
&& 8    & 4.65    & 10.00  \\  
&& 6    & 6.35    & 64.06  \\  
&& 5    & 7.84    & 64.19  \\  
&& 4    & 10.09    & 64.02  \\  
&& 3    & 14.09    & 64.87  \\  
&& 2    & 24.01    & 64.93  \\  
&& 1    & 61.51    & 64.99  \\ 

\midrule


\multirow{5}{*}{\makecell{\\ \\ \\Imagenette }}&
\multirow{5}{*}{\makecell{\\ \\ \\ 0.7  }}&

30      & 1.16    & 9.86  \\  
&& 25    & 1.40    & 9.86  \\  
&& 20    & 1.76    & 9.86  \\  
&& 15    & 2.37    & 29.36  \\  
&& 10    & 3.64    & 74.75  \\  
&& 8    & 4.65    & 75.03  \\  
&& 6    & 6.35    & 76.37  \\  
&& 1    & 61.51    & 76.55  \\ 

\midrule


\multirow{5}{*}{\makecell{\\ \\ \\NUS-WIDE }}&
\multirow{5}{*}{\makecell{\\ \\ \\ 0.3  }}&

30      & 1.16    & 82.89  \\  
&& 25    & 1.40    & 83.14  \\  
&& 20    & 1.76    & 83.17  \\  
&& 15    & 2.35    & 83.00  \\  
&& 10    & 3.64    & 83.25  \\  
&& 8    & 4.65    & 82.88  \\  
&& 6    & 6.35    & 82.71  \\  
&& 1    & 61.51    & 83.14  \\ 



\bottomrule
\end{tabular}
}
}


==> tables/single_attacker.tex <==
\resizebox{\textwidth}{!}{
{
% \scriptsize
% \begin{tabular}{TCC|AAAAAA|AAAAAA|AAAAAD}
\renewcommand{\arraystretch}{1.0}
% \begin{tabular}{TTT|CCCCCC|CCCCCD}
\begin{tabular}{TCCAAAAAA|AAAAAD}
     \toprule
        \multirow{3}{*}[-1em]{Dataset} & \multirow{3}{*}[-0.8em]{\makecell{Label\\ Knowledge}} & \multirow{3}{*}[-1em]{Attack} & \multicolumn{12}{c}{Defense} \\

        
        \cmidrule(lr){4-15}  
        
        {} & {} & {} & \multicolumn{6}{c}{Accuracy (\%) $\uparrow$  \text{(Higher is better)}} & \multicolumn{6}{c}{Attack Success Rate (\%) $\downarrow$ \text{(Lower is better)}} 
        % \multicolumn{6}{c}{Robust Accuracy (\%) $\uparrow$  \text{(Higher is better)}} 
        \\
        \cmidrule(lr){4-9} \cmidrule(lr){10-15} 
        % \cmidrule(lr){16-21}
        
        {} & {} & {} & NO DEF & DP-SGD & MP  & ANP & BDT  & VFLIP & NO DEF & DP-SGD & MP  & ANP & BDT  & VFLIP \\
        % & 
        % NO DEF & DP-SGD & MP  & ANP & BDT  & VFLIP \\
        \midrule

        %% CIFAR10
        \multirow{4}{*}[-0.3em]{CIFAR10}  & \multirow{2}{*}{w/o}  & BadVFL 
        &77.34	&\textbf{78.04}	&75.35	&75.53	&73.28	&75.14	
        &30.58	&30.81	&25.55	&28.14	&29.20	&\textbf{13.95}
        % & 59.78	&53.51	&49.80	&55.62	&53.21	&\textbf{64.14} 
        \\

        {} & {}  & VILLIAN 
        &\textbf{76.84}	&75.04	&75.34	&73.40	&73.15	&75.22	
        &86.96	&20.40	&79.17	&64.83	&83.00	&\textbf{3.19}
        % & 24.36	&60.09	&31.40	&31.61	&29.07	&\textbf{68.58} 
        \\
        \cmidrule{2-15}
        
        {} & \multirow{2}{*}{with}  & BadVFL 
        &76.85	&\textbf{77.30}	&74.83	&75.41	&72.46	&75.46	
        &97.50	&99.99	&87.13	&96.49	&95.51	&\textbf{5.52}
        % & 10.60	&10.02	&20.94	&15.66	&14.27	&\textbf{65.30} 
        \\

        {} & {}  & VILLIAN 
        &75.46	&\textbf{75.52}	&74.94	&74.11	&74.33	&73.86	
        &99.84	&64.13	&99.76	&99.80	&99.77	&\textbf{2.79}
        % & 10.09	&41.70	&10.44	&10.18	&10.18	&\textbf{66.71} 
        \\




        %% CINIC10L
        \midrule 
        \multirow{4}{*}[-0.3em]{CINIC10}  & \multirow{2}{*}{w/o}  & BadVFL 
        &\textbf{64.60}	&64.43	&64.37	&64.34	&61.94	&62.45	
        &21.13	&28.27	&18.05	&17.89	&19.52	&\textbf{13.90}
        % &53.14	&50.59	&54.69	&\textbf{56.15}	&54.17	&54.85 
        \\

        {} & {}  & VILLIAN 
        &\textbf{63.66}	&63.14	&63.30	&63.33	&60.88	&62.27	
        &75.65	&11.53	&64.30	&65.03	&70.36	&\textbf{3.74}
        % &27.45	&54.61	&25.11	&28.43	&25.18	&\textbf{57.00} 
        \\
        \cmidrule{2-15}
        
        {} & \multirow{2}{*}{with}  & BadVFL 
        &\textbf{64.37}	&62.46	&62.22	&63.88	&60.40	&63.21	
        &99.46	&80.31	&91.51	&96.82	&99.25	&\textbf{4.92}
        % &10.01	&10.01	&10.22	&10.26	&10.31	&\textbf{56.11} 
        \\

        {} & {}  & VILLIAN 
        &\textbf{62.43}	&61.73	&61.93	&62.09	&60.91	&61.05	
        &99.97	&85.41	&99.91	&99.94	&99.97	&\textbf{2.34}
        % & 10.00	&14.97	&10.00	&10.01	&10.01	&\textbf{55.72}
        \\


        %% Imagenette
        \midrule 
        \multirow{4}{*}[-0.3em]{Imagenette} & \multirow{2}{*}{w/o}  & BadVFL 
        &\textbf{75.48}	&74.98	&72.54	&75.07	&71.22	&73.37	
        &61.02	&78.01	&54.37	&60.21	&58.46	&\textbf{14.41}
        % &27.73	&63.09	&27.54	&28.21	&28.72	&\textbf{66.60} 
        \\

        {} & {}  & VILLIAN 
        &\textbf{74.11}	&73.83	&72.55	&73.12	&71.25	&71.60	
        &96.66	&23.80	&93.95	&96.50	&96.50	&\textbf{2.87}
        % &14.68	&42.17	&19.97	&15.81	&15.81	&\textbf{67.17} 
        \\
        \cmidrule{2-15}
        
        {} & \multirow{2}{*}{with}  & BadVFL 
        &74.02	&\textbf{74.97}	&70.84	&73.64	&69.43	&71.70	
        &92.21	&93.20	&73.36	&92.08	&90.62	&\textbf{3.79}
        % &13.05	&18.80	&12.48	&11.22	&11.95	&\textbf{63.06} 
        \\

        {} & {}  & VILLIAN 
        &72.31	&\textbf{73.27}	&69.50	&71.37	&69.45	&69.32	
        &97.38	&89.29	&96.70	&97.33	&97.42	&\textbf{1.87}
        % & 11.89	&15.53	&12.16	&10.50	&10.71	&\textbf{64.21} 
        \\


        %% NUS-WIDE
        \midrule 
        \multirow{4}{*}[-0.3em]{NUS-WIDE} & \multirow{2}{*}{w/o}  & BadVFL 
        &\textbf{83.55}	&83.32	&82.99	&81.42	&81.66	&81.26	
        &72.65	&57.68	&68.66	&61.82	&73.12	&\textbf{9.28}
        % & 39.62	&51.37	&41.62	&63.85	&40.29	&\textbf{70.86}
        \\

        {} & {}  & VILLIAN 
        &\textbf{83.74}	&83.16	&81.78	&80.75	&81.21	&81.39	
        &89.34	&23.73	&80.13	&72.33	&88.75	&\textbf{7.65}
        % & 33.97	&60.43	&31.26	&67.40	&26.83	&\textbf{71.52} 
        \\
        \cmidrule{2-15}
        
        {} & \multirow{2}{*}{with}  & BadVFL 
        &\textbf{82.79}	&81.45	&80.72	&82.52	&81.76	&79.93	
        &99.99	&95.55	&95.11	&99.98	&99.97	&\textbf{12.45}
        % & 19.92	&20.14	&19.95	&19.95	&20.02	&\textbf{69.42} 
        \\

        {} & {}  & VILLIAN 
        &\textbf{82.44}	&80.50	&80.47	&79.26	&80.68	&80.51	
        &100.00	&96.75	&99.91	&99.22	&100.00	&\textbf{6.30}
        % & 19.91	&22.45	&19.92	&19.91	&19.91	&\textbf{72.48} 
        \\


        %% BM
        \midrule 
        \multirow{4}{*}[-0.3em]{BM} & \multirow{2}{*}{w/o}  & BadVFL 
        &\textbf{83.55}	&83.32	&82.99	&81.42	&81.66	&81.26	
        &72.65	&57.68	&68.66	&61.82	&73.12	&\textbf{9.28}
        % & 39.62	&51.37	&41.62	&63.85	&40.29	&\textbf{70.86}
        \\

        {} & {}  & VILLIAN 
        &\textbf{83.74}	&83.16	&81.78	&80.75	&81.21	&81.39	
        &89.34	&23.73	&80.13	&72.33	&88.75	&\textbf{7.65}
        % & 33.97	&60.43	&31.26	&67.40	&26.83	&\textbf{71.52} 
        \\
        \cmidrule{2-15}
        
        {} & \multirow{2}{*}{with}  & BadVFL 
        &\textbf{82.79}	&81.45	&80.72	&82.52	&81.76	&79.93	
        &99.99	&95.55	&95.11	&99.98	&99.97	&\textbf{12.45}
        % & 19.92	&20.14	&19.95	&19.95	&20.02	&\textbf{69.42} 
        \\

        {} & {}  & VILLIAN 
        &\textbf{82.44}	&80.50	&80.47	&79.26	&80.68	&80.51	
        &100.00	&96.75	&99.91	&99.22	&100.00	&\textbf{6.30}
        % & 19.91	&22.45	&19.92	&19.91	&19.91	&\textbf{72.48} 
        \\

        \bottomrule

\end{tabular}
}
}
